A Survey of AI-Powered Mini-Grid Solutions for a Sustainable Future in Rural Communities

This paper presents a comprehensive survey of AI-driven mini-grid solutions aimed at enhancing sustainable energy access. It emphasises the potential of mini-grids, which can operate independently or in conjunction with national power grids, to provide reliable and affordable electricity to remote communities. Given the inherent unpredictability of renewable energy sources such as solar and wind, the necessity for accurate energy forecasting and management is discussed, highlighting the role of advanced AI techniques in forecasting energy supply and demand, optimising grid operations, and ensuring sustainable energy distribution. This paper reviews various forecasting models, including statistical methods, machine learning algorithms, and hybrid approaches, evaluating their effectiveness for both short-term and long-term predictions. Additionally, it explores public datasets and tools such as Prophet, NeuralProphet, and N-BEATS for model implementation and validation. The survey concludes with recommendations for future research, addressing challenges in model adaptation and optimisation for real-world applications.

==> next_steps.tex <==
\section{Next Steps}

The work presented in this report serves as a precursor to the implementation of the proposed mini-grid in Work Package 2, as well as the development of suitable AI forecasting models for Work Package 3. An overview of the aforementioned Work Packages is detailed below.

\textbf{WP2}: Design and installation of an experimental mini-grid that uses solar and wind as the primary energy sources together with a battery backup and a standby diesel generator.

\textbf{WP3}: Development and testing of an AI-powered mini-grid management system that optimises the
key technical operations of the proposed mini-grid by improving the balancing of generation, storage, 
distribution and consumption of electricity. From an analysis of the techniques described within this Work Package, WP3 will initially involve a greater exploration of the test data-set to determine patterns and correlations within the data.
